What Makes for Text to 360-degree Panorama Generation with Stable Diffusion?

Recent prosperity of text-to-image diffusion models, e.g. Stable Diffusion, has stimulated research to adapt them to 360-degree panorama generation. Prior work has demonstrated the feasibility of using conventional low-rank adaptation techniques on pre-trained diffusion models to generate panoramic images. However, the substantial domain gap between perspective and panoramic images raises questions about the underlying mechanisms enabling this empirical success. We hypothesize and examine that the trainable counterparts exhibit distinct behaviors when fine-tuned on panoramic data, and such an adaptation conceals some intrinsic mechanism to leverage the prior knowledge within the pre-trained diffusion models. Our analysis reveals the following: 1) the query and key matrices in the attention modules are responsible for common information that can be shared between the panoramic and perspective domains, thus are less relevant to panorama generation; and 2) the value and output weight matrices specialize in adapting pre-trained knowledge to the panoramic domain, playing a more critical role during fine-tuning for panorama generation. We empirically verify these insights by introducing a simple framework called UniPano, with the objective of establishing an elegant baseline for future research. UniPano not only outperforms existing methods but also significantly reduces memory usage and training time compared to prior dual-branch approaches, making it scalable for end-to-end panorama generation with higher resolution. The code will be released.

==> preamble.tex <==
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}

\usepackage{booktabs}
\usepackage{overpic}
\usepackage{amssymb,amsfonts,amsmath,amssymb,endnotes,rotating,arydshln}
\usepackage{mathrsfs}
\usepackage{bm,pifont}
% \usepackage[nohead]{geometry}
% \usepackage[singlespacing]{setspace}
% \usepackage[bottom]{footmisc}
% \usepackage{graphicx,array,booktabs,bbm}
% \RequirePackage[OT1]{fontenc} 
\RequirePackage{amsthm,amsmath}
\usepackage{thmtools,thm-restate}
\usepackage[numbers,sort&compress]{natbib}
% \RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{comment}

\usepackage{caption}
\usepackage{cuted}
\usepackage[normalem]{ulem}

\def\Jing#1{{\color{magenta}{\bf [Jing:} {\it{#1}}{\bf ]}}}


% \usepackage{subfigure}
% \graphicspath{ {./images/} }
% \usepackage{float}
% \renewcommand\thefigure{\arabic{figure}}
% \setcounter{figure}{1}

% \usepackage[ruled,vlined]{algorithm2e}
% \usepackage{algorithm}% http://ctan.org/pkg/algorithms
% \usepackage[algcompatible]{algpseudocode}% http://ctan.org/pkg/algorithmicx
\newcommand{\algvar}[1]{{\ttfamily#1}}% variable
\usepackage{multirow}
\usepackage{subcaption}

\usepackage{bbding}

\usepackage[table]{xcolor}


% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{fact}[theorem]{Fact}
% \newtheorem{assumption}[theorem]{Assumption}
% \newtheorem{remark}{Remark}[section]
% \newtheorem{observation}{Observation}[section]
% \newtheorem{conclusion}{Conclusion}[section]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{conclusion}[theorem]{Conclusion}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\usepackage{mathtools}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}
\newcommand{\mtx}[1]{\bm{#1}}
\newcommand{\Prob}[1]{\mathbb{P}\left\{ {#1} \right\}}
\newcommand{\Expect}{\operatorname{\mathbb{E}}}
\newcommand{\psdle}{\preccurlyeq}
\newcommand{\psdge}{\succcurlyeq}
\newcommand{\econst}{\mathrm{e}}
\newcommand{\adj}{*}

\newcommand{\field}[1]{\mathbb{#1}}
\newcommand{\R}{\field{R}}
\newcommand{\F}{\field{F}}
\newcommand{\p}{\field{P}}
\newcommand{\N}{\field{N}}
\newcommand{\Z}{\field{Z}}
\newcommand{\X}{\field{X}}
\newcommand{\E}{\field{E}}
\def\qed{\hfill$\diamondsuit$}
\def\II{I\negthinspace I}
\def\B{I\negthinspace\negthinspace B}
\def\ccirc{\negthinspace\circ}
% \newcommand{\rmnum}[1]{\romannumeral #1}
% \newcommand{\Rmnum}[1]{\expandafter\romannumeral #1}
\newcommand*{\I}{\imath}
\def\cod{\stackrel{\cal D}{\longrightarrow}}
\def\cop{\stackrel{\cal P}{\longrightarrow}}
\def\eqd{\stackrel{\cal D}{=}}
\def\eqp{\stackrel{\cal P}{=}}
\def\ap#1{\smash{\mathop{\approx}\limits^{#1}}}
\def\lf{\lfloor}
\def\rf{\rfloor}
\def\lc{\lceil}
\def\rc{\rceil}
% \font\n=cmcsc12
\def\cov{{\mbox{cov}}}
\def\corr{{\mbox{corr}}}
\def\var{{\mbox{var}}}
\def\cum{{\mbox{cum}}}
\def\Z{{\mathcal{Z}}}

% \makeatletter \makeatother
% \textwidth = 420pt
% \geometry{left=1in,right=1in,top=1.25in,bottom=1.0in}
% \renewcommand{\baselinestretch}{1.3}

\newcommand{\dotp}[2]{\left\langle #1, #2\right\rangle}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\Var}{\mathop{\rm Var}}
\newcommand{\Cov}{\mathop{\rm Cov}}
\newcommand{\dom}{\mathop{\rm dom} \,}

\newcommand{\bfY} {\mbox{\boldmath $Y$}}
% \newcommand{\bfX} {\mbox{\boldmath $X$}}
\newcommand{\bfX}{{\bf X}}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfk}{{\bf k}}
\newcommand{\bfK}{{\bf K}}
\newcommand{\ci}{\mid\mid}

\newcommand{\ve}{\varepsilon}

\newcommand{\bfth} {\mbox{\boldmath $\theta$}}
\newcommand{\bfgam} {\mbox{\boldmath $\gamma$}}
\newcommand{\bfe} {\mbox{\boldmath $\epsilon$}}
\newcommand{\bfeb} {\mbox{\boldmath $\underline{\epsilon}$}}
\newcommand{\bfxi} {\mbox{\boldmath $\xi$}}
\newcommand{\bfph} {\mbox{\boldmath $\phi$}}
\newcommand{\bfPh} {\mbox{\boldmath $\Phi$}}

\newcommand{\wt}{\widetilde}
\newcommand{\wht}{\widehat}
\usepackage{amsmath}

\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\seq}[1]{\left<#1\right>}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\brkt}[1]{\left[#1\right]}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\essnorm}[1]{\norm{#1}_{\ess}}
\newcommand{\dd}{{\mathrm d}}
\newcommand \bbP{\mathbb{P}}
\newcommand \bbE{\mathbb{E}}
\newcommand \bbR{\mathbb{R}}
\newcommand \bbL{\mathbb{L}}

%\newcommand{\cmi}{\mbox{i}}
\def\m{\mathcal}
\def\ms{\mathscr}
\def\mb{\mathbb}
\def\mr{\mathrm}
\def\mx{\mbox}
\def\Gauss{{ \mathrm{N} }}
\newcommand{\ind}{\mathbbm{1}}

\def\T{{ \mathrm{\scriptscriptstyle T} }}
\def\ADG{\textcolor{magenta}} % leave comments

\def \nystrom {{Nystr\"{o}m }}
\def \matern {{Mat\'{e}rn }}
\def \holder {{H\"{o}lder}}


% Uschi's macros

\newcommand{\bmp}{\begin{minipage}}
\newcommand{\emp}{\end{minipage}}
\newcommand{\ben}{\begin{eqnarray*}}
\newcommand{\non}{\end{eqnarray*}}
\newcommand{\1}{\\[1ex]}
\newcommand{\2}{\\[2ex]}
\newcommand{\3}{\\[3ex]}
\newcommand{\4}{\\[4ex]}
\newcommand{\cS}{{\cal S}}
\newcommand{\A}{{\cal A}}
\newcommand{\0}{\emptyset}
\newcommand{\si}{\sum_{i=1}^n}
\newcommand{\avi}{\frac 1 n \si}
\newcommand{\sj}{\sum_{j=1}^n}
\newcommand{\cupi}{\cup_{i=1}^n}
\newcommand{\capi}{\cap_{i=1}^n}
\newcommand{\ds}{\displaystyle}
%\newcommand{\n}{\noindent}
\newcommand{\real}{\ensuremath{\mathbb R}}
\newcommand{\nat}{\ensuremath{\mathbb N}}
%\renewcommand{\baselinestretch}{0.98}
\newcommand{\darrow}{\stackrel{\cal D}{\longrightarrow} }
\newcommand{\parrow}{\stackrel{P}{\rightarrow} }
\newcommand{\nn}{\newpage \noindent}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}

\usepackage{enumitem}
\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0.5pt] (char) {#1};}}

\makeatletter
\newcommand*{\Rom}[1]{\expandafter\@slowromancap\romannumeral #1@}
\newcommand*{\rom}[1]{\romannumeral#1\relax}
% \uppercase\expandafter{\romannumeral<number>\relax}
\makeatother
% \usepackage{xr}

% \input{math_commands.tex}


\newcommand{\rb}[1]{\left( #1 \right)}
\newcommand{\h}[1]{\hat{#1}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\mcal}[1]{\mathcal{#1}}
\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}

\newcommand{\njh}[1]{\textcolor{cyan}{[JH: #1]}}

% Include other packages here, before hyperref.

% If you comment hyperref and then uncomment it, you should delete
% egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% run, let it finish, and you should be clear).
% \usepackage[breaklinks=true,bookmarks=false]{hyperref}




\captionsetup{skip=2pt}
\setlength{\textfloatsep}{8.0pt plus 2.0pt minus 4.0pt}
\setlength{\floatsep}{8.0pt plus 2.0pt minus 2.0pt}
\setlength{\intextsep}{8.0pt plus 2.0pt minus 2.0pt}
\setlength{\dbltextfloatsep}{8.0pt plus 2.0pt minus 2.0pt}
\setlength{\dblfloatsep}{8.0pt plus 2.0pt minus 2.0pt}
